FIRST: Teach A Reliable Large Language Model Through Efficient Trustworthy Distillation

Large language models (LLMs) have become increasingly prevalent in our daily lives, leading to an expectation for LLMs to be trustworthy -- - both accurate and well-calibrated (the prediction confidence should align with its ground truth correctness likelihood). Nowadays, fine-tuning has become the most popular method for adapting a model to practical usage by significantly increasing accuracy on downstream tasks. Despite the great accuracy it achieves, we found fine-tuning is still far away from satisfactory trustworthiness due to "tuning-induced mis-calibration". In this paper, we delve deeply into why and how mis-calibration exists in fine-tuned models, and how distillation can alleviate the issue. Then we further propose a brand new method named Efficient Trustworthy Distillation (FIRST), which utilizes a small portion of teacher's knowledge to obtain a reliable language model in a cost-efficient way. Specifically, we identify the "concentrated knowledge" phenomenon during distillation, which can significantly reduce the computational burden. Then we apply a "trustworthy maximization" process to optimize the utilization of this small portion of concentrated knowledge before transferring it to the student. Experimental results demonstrate the effectiveness of our method, where better accuracy (+2.3%) and less mis-calibration (-10%) are achieved on average across both in-domain and out-of-domain scenarios, indicating better trustworthiness.

==> Figures/coefficient.tex <==
\begin{table*}[!t]
\footnotesize
\centering
    \caption{123}
    \label{tab:main_result}

    \vskip 0.15in
    \begin{tabular}{l|cccc|cccc}
    \toprule
    
     
     Coefficient &  0.1 & 0.3 & 0.5 & 0.7\\
     
     &\multicolumn{2}{c}{Commonsense QA}& \multicolumn{2}{c}{BoolQ} &\multicolumn{2}{c}{Alpaca $\rightarrow$ Commonsense QA}& \multicolumn{2}{c}{Alpaca $\rightarrow$ OBQA}\\
     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
      & ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ \\
      \midrule
     & \multicolumn{8}{c}{\textsc{Llama-33B $\rightarrow$ Llama-7B}}\\
     \midrule
     Pre-train\textsubscript{ 7B} & 0.042 & 28.1\% & 0.425 & 61.3\% & 0.039 & 27.8\% & 0.04 & 27.2\% \\
     Teacher\textsubscript{ 33B} & \gray{0.102} & \gray{82.4\%} & \gray{0.077} & \gray{89.7\%} & \gray{0.186} & \gray{69.2\%} & \gray{0.202} & \gray{64.4\%} \\
     Fine-tune\textsubscript{ 7B} & 0.118 & 79.9\% & 0.065 & 82.5\% & 0.125 & 48.2\% & 0.219 & 43.4\% \\
     Distill\textsubscript{ 7B w/o Calibration} & 0.094 & 78.9\% & \textbf{0.04} & 85.3\% & 0.053 & 43.1\% & 0.181 & 39.8\% \\
     Distill\textsubscript{ 7B w/ Label Smoothing} & 0.091 & 78.1\% & 0.190 & 85.3\% & 0.052 & 43.9\% & 0.19 & 37.6\% \\
     Distill\textsubscript{ 7B w/ ODR} & \textbf{0.029} & \textbf{80.8\%} & \textbf{0.04} & \textbf{85.7\%} & \textbf{0.046} & \textbf{50.0\%} &\textbf{ 0.071} & \textbf{47.2\%} \\
     Compare to w/o calibration& $\red{\uparrow_{6.5\%}}$ & $\red{\uparrow_{1.9\%}}$ & $\blue{\uparrow_{0\%}}$ & $\red{\uparrow_{0.4\%}}$ & $\red{\uparrow_{0.7\%}}$ & $\red{\uparrow_{6.9\%}}$ & $\red{\uparrow_{11\%}}$ & $\red{\uparrow_{7.4\%}}$\\
    
     \midrule
     & \multicolumn{8}{c}{\textsc{Llama-2-13B $\rightarrow$ Llama-2-7B}}\\
     \midrule
     Pre-train\textsubscript{ 7B} & 0.1 & 36.6\% & 0.386 & 57.2\% & 0.1 & 36.6\% & 0.125 & 44.7\% \\
     Teacher\textsubscript{ 13B} & \gray{0.12} & \gray{81.6\%} & \gray{0.068} & \gray{89.7\%} & \gray{0.208} & \gray{65.7\%} & \gray{0.287} & \gray{58.3\%} \\
     Fine-tune\textsubscript{ 7B} & 0.14 & 76.8\% & 0.084 & 87.5\% & 0.212 & 50.0\% & 0.301 & 45.6\% \\
     Distill\textsubscript{ 7B w/o Calibration} & 0.109 & 80.0\% & 0.04 & 85.3\% & 0.077 & 50.9\% & 0.125 & 46.6\% \\
     Distill\textsubscript{ 7B w/ Label Smoothing} & 0.103 & \textbf{80.4\%} & 0.039 & 87.5\% & 0.075 & 51.1\% & 0.162 & 47.6\%\\
     Distill\textsubscript{ w/ ODR} & \textbf{0.063} & 80.3\% & \textbf{0.014} & \textbf{87.9\%} & \textbf{0.055} & \textbf{51.4\%} & \textbf{0.081} & \textbf{49.5\%} \\
     Compare to w/o calibration& $\red{\uparrow_{4.6\%}}$ & $\red{\uparrow_{0.3\%}}$ & $\red{\uparrow_{2.6\%}}$ & $\red{\uparrow_{2.6\%}}$ & $\red{\uparrow_{2.2\%}}$ & $\red{\uparrow_{0.5\%}}$ & $\red{\uparrow_{4.4\%}}$ & $\red{\uparrow_{2.9\%}}$\\
     \midrule
     & \multicolumn{8}{c}{\textsc{OpenLlama-13B $\rightarrow$ OpenLlama-7B}}\\
     \midrule
     Pre-train\textsubscript{ 7B} & 0.075 & 20.8\% & 0.359 & 58.5\% & 0.075 & 20.8\% & 0.008 & 28.4\% \\
     Teacher\textsubscript{ 13B} & \gray{0.132} & \gray{78.5\%} & \gray{0.075} & \gray{87.6} & \gray{0.167} & \gray{49.5\%} & \gray{0.134} & \gray{50\%} \\
     Fine-tune\textsubscript{ 7B} & 0.105 & 75.0\% & 0.036 & 81.5\% & 0.216 & 28.3\% & 0.161 & 30.4\% \\
     Distill\textsubscript{ 7B w/o Calibration} & 0.092 & 75.2\% & 0.062 & 83.8\% & 0.097 & 27.7\% & 0.137 & 29.8\% \\
     Distill\textsubscript{ 7B w/ Label Smoothing} & 0.096 & 74.5\% & 0.033 & 83.3\% & 0.041 & 29.2\% & 0.142 & 29.8\% \\
     Distill\textsubscript{ 7B w/ ODR} & \textbf{0.050} & \textbf{77.2\%} &\textbf{ 0.027} & \textbf{84.7\%} & \textbf{0.029} & \textbf{30.5\%} & \textbf{0.082} & \textbf{30.8\%} \\
     Compare to w/o calibration& $\red{\uparrow_{4.2\%}}$ & $\red{\uparrow_{2.0\%}}$ & $\red{\uparrow_{3.5\%}}$ & $\red{\uparrow_{0.9\%}}$ & $\red{\uparrow_{6.8\%}}$ & $\red{\uparrow_{2.8\%}}$ & $\red{\uparrow_{5.5\%}}$ & $\red{\uparrow_{1.0\%}}$\\

    \bottomrule
    % & \multicolumn{10}{c}{\textbf{Forgetting}}
    % & 
    \end{tabular}

\end{table*}
% $\red{\uparrow}$ means the improvement of distilled models over fine-tuned small models.

==> Tables/NOT_USED_omer_table_2.tex <==
\begin{table*}[!t]
\footnotesize
\centering
    % \vskip 0.15in
    \begin{tabular}{l|cccc|}
    \toprule

     
     & \multicolumn{4}{c}{\textsc{\textbf{In-Domain}}} \\
     
     &\multicolumn{2}{c}{Commonsense QA}& \multicolumn{2}{c}{BoolQ} \\
     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
      & ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ \\
      \midrule
     & \multicolumn{4}{c}{\textsc{Llama 1 : 33B $\rightarrow$ 7B}}\\
     \midrule
     Pre-train\textsubscript{ 7B} & 0.042 & 28.1\% & 0.425 & 61.3\% \\
     Teacher\textsubscript{ 33B} & \gray{0.102} & \gray{82.4\%} & \gray{0.077} & \gray{89.7\%} \\
     Fine-tune\textsubscript{ 7B} & 0.118 & 79.9\% & 0.065 & 82.5\% \\
     Distill\textsubscript{ 7B w/o Re-calibration} & 0.094 & 78.9\% & \textbf{0.04} & 85.3\% \\
     Distill\textsubscript{ 7B w/ Label Smoothing} & 0.091 & 78.1\% & 0.190 & 85.3\% \\
     Distill\textsubscript{ 7B w/ COD} & \textbf{0.029} & \textbf{80.8\%} & \textbf{0.04} & \textbf{85.7\%} \\
     COD to w/o Re-calibration& $\red{\uparrow_{6.5\%}}$ & $\red{\uparrow_{1.9\%}}$ & $\blue{\uparrow_{0\%}}$ & $\red{\uparrow_{0.4\%}}$ \\
    
     \midrule
     & \multicolumn{4}{c}{\textsc{Llama 2 : 13B$^*$ $\rightarrow$ 7B}}\\
     \midrule
     Pre-train\textsubscript{ 7B} & 0.1 & 36.6\% & 0.386 & 57.2\% \\
     Teacher\textsubscript{ 13B} & \gray{0.12} & \gray{81.6\%} & \gray{0.068} & \gray{89.7\%} \\
     Fine-tune\textsubscript{ 7B} & 0.14 & 76.8\% & 0.084 & 87.5\% \\
     Distill\textsubscript{ 7B w/o Re-calibration} & 0.109 & 80.0\% & 0.04 & 85.3\% \\
     Distill\textsubscript{ 7B w/ Label Smoothing} & 0.103 & \textbf{80.4\%} & 0.039 & 87.5\% \\
     Distill\textsubscript{ w/ COD} & \textbf{0.063} & 80.3\% & \textbf{0.014} & \textbf{87.9\%} \\
     COD to w/o Re-calibration& $\red{\uparrow_{4.6\%}}$ & $\red{\uparrow_{0.3\%}}$ & $\red{\uparrow_{2.6\%}}$ & $\red{\uparrow_{2.6\%}}$ \\
     \midrule
     & \multicolumn{4}{c}{\textsc{OpenLlama : 13B $\rightarrow$ 7B}}\\
     \midrule
     Pre-train\textsubscript{ 7B} & 0.075 & 20.8\% & 0.359 & 58.5\% \\
     Teacher\textsubscript{ 13B} & \gray{0.132} & \gray{78.5\%} & \gray{0.075} & \gray{87.6} \\
     Fine-tune\textsubscript{ 7B} & 0.105 & 75.0\% & 0.036 & 81.5\% \\
     Distill\textsubscript{ 7B w/o Re-calibration} & 0.092 & 75.2\% & 0.062 & 83.8\% \\
     Distill\textsubscript{ 7B w/ Label Smoothing} & 0.096 & 74.5\% & 0.033 & 83.3\% \\
     Distill\textsubscript{ 7B w/ COD} & \textbf{0.050} & \textbf{77.2\%} &\textbf{ 0.027} & \textbf{84.7\%} \\
     COD to w/o Re-calibration& $\red{\uparrow_{4.2\%}}$ & $\red{\uparrow_{2.0\%}}$ & $\red{\uparrow_{3.5\%}}$ & $\red{\uparrow_{0.9\%}}$ \\

    \bottomrule
    % & \multicolumn{10}{c}{\textbf{Forgetting}}
    % & 
    \end{tabular}
    \caption{The overall experimental results of calibration and performance on downstream tasks under both in-domain and out-of-domain setting. We compare pre-trained models, fine-tuned teacher and student models, and distilled models w/ or w/o re-calibration. The $\uparrow$ represents the larger the better while the $\downarrow$ means the smaller the better. \textbf{Bold} represents the best among fine-tuned and distilled student models. \gray{Gray} represents the statistics presented are for reference only and should not be used for comparison purposes. The model sizes are all specified in the subscripts. $^*$: We use 13B teacher model for Llama 2 family as its 34B version is still not publicly available and its 70B version requires significantly more resources. }
    \label{tab:main_result}
    \vskip -0.2in

\end{table*}
% $\red{\uparrow}$ means the improvement of distilled models over fine-tuned small models.





==> Tables/coefficient.tex <==
\begin{table*}[!t]
\footnotesize
\centering
    \caption{123}
    \label{tab:main_result}

    \vskip 0.15in
    \begin{tabular}{l|cccc|cccc}
    \toprule
    
     
     Coefficient &  0.1 & 0.3 & 0.5 & 0.7\\
     
     &\multicolumn{2}{c}{Commonsense QA}& \multicolumn{2}{c}{BoolQ} &\multicolumn{2}{c}{Alpaca $\rightarrow$ Commonsense QA}& \multicolumn{2}{c}{Alpaca $\rightarrow$ OBQA}\\
     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
      & ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ \\
      \midrule
     & \multicolumn{8}{c}{\textsc{Llama-33B $\rightarrow$ Llama-7B}}\\
     \midrule
     Pre-train\textsubscript{ 7B} & 0.042 & 28.1\% & 0.425 & 61.3\% & 0.039 & 27.8\% & 0.04 & 27.2\% \\
     Teacher\textsubscript{ 33B} & \gray{0.102} & \gray{82.4\%} & \gray{0.077} & \gray{89.7\%} & \gray{0.186} & \gray{69.2\%} & \gray{0.202} & \gray{64.4\%} \\
     Fine-tune\textsubscript{ 7B} & 0.118 & 79.9\% & 0.065 & 82.5\% & 0.125 & 48.2\% & 0.219 & 43.4\% \\
     Distill\textsubscript{ 7B w/o Calibration} & 0.094 & 78.9\% & \textbf{0.04} & 85.3\% & 0.053 & 43.1\% & 0.181 & 39.8\% \\
     Distill\textsubscript{ 7B w/ Label Smoothing} & 0.091 & 78.1\% & 0.190 & 85.3\% & 0.052 & 43.9\% & 0.19 & 37.6\% \\
     Distill\textsubscript{ 7B w/ COD} & \textbf{0.029} & \textbf{80.8\%} & \textbf{0.04} & \textbf{85.7\%} & \textbf{0.046} & \textbf{50.0\%} &\textbf{ 0.071} & \textbf{47.2\%} \\
     Compare to w/o calibration& $\red{\uparrow_{6.5\%}}$ & $\red{\uparrow_{1.9\%}}$ & $\blue{\uparrow_{0\%}}$ & $\red{\uparrow_{0.4\%}}$ & $\red{\uparrow_{0.7\%}}$ & $\red{\uparrow_{6.9\%}}$ & $\red{\uparrow_{11\%}}$ & $\red{\uparrow_{7.4\%}}$\\
    
     \midrule
     & \multicolumn{8}{c}{\textsc{Llama-2-13B $\rightarrow$ Llama-2-7B}}\\
     \midrule
     Pre-train\textsubscript{ 7B} & 0.1 & 36.6\% & 0.386 & 57.2\% & 0.1 & 36.6\% & 0.125 & 44.7\% \\
     Teacher\textsubscript{ 13B} & \gray{0.12} & \gray{81.6\%} & \gray{0.068} & \gray{89.7\%} & \gray{0.208} & \gray{65.7\%} & \gray{0.287} & \gray{58.3\%} \\
     Fine-tune\textsubscript{ 7B} & 0.14 & 76.8\% & 0.084 & 87.5\% & 0.212 & 50.0\% & 0.301 & 45.6\% \\
     Distill\textsubscript{ 7B w/o Calibration} & 0.109 & 80.0\% & 0.04 & 85.3\% & 0.077 & 50.9\% & 0.125 & 46.6\% \\
     Distill\textsubscript{ 7B w/ Label Smoothing} & 0.103 & \textbf{80.4\%} & 0.039 & 87.5\% & 0.075 & 51.1\% & 0.162 & 47.6\%\\
     Distill\textsubscript{ w/ COD} & \textbf{0.063} & 80.3\% & \textbf{0.014} & \textbf{87.9\%} & \textbf{0.055} & \textbf{51.4\%} & \textbf{0.081} & \textbf{49.5\%} \\
     Compare to w/o calibration& $\red{\uparrow_{4.6\%}}$ & $\red{\uparrow_{0.3\%}}$ & $\red{\uparrow_{2.6\%}}$ & $\red{\uparrow_{2.6\%}}$ & $\red{\uparrow_{2.2\%}}$ & $\red{\uparrow_{0.5\%}}$ & $\red{\uparrow_{4.4\%}}$ & $\red{\uparrow_{2.9\%}}$\\
     \midrule
     & \multicolumn{8}{c}{\textsc{OpenLlama-13B $\rightarrow$ OpenLlama-7B}}\\
     \midrule
     Pre-train\textsubscript{ 7B} & 0.075 & 20.8\% & 0.359 & 58.5\% & 0.075 & 20.8\% & 0.008 & 28.4\% \\
     Teacher\textsubscript{ 13B} & \gray{0.132} & \gray{78.5\%} & \gray{0.075} & \gray{87.6} & \gray{0.167} & \gray{49.5\%} & \gray{0.134} & \gray{50\%} \\
     Fine-tune\textsubscript{ 7B} & 0.105 & 75.0\% & 0.036 & 81.5\% & 0.216 & 28.3\% & 0.161 & 30.4\% \\
     Distill\textsubscript{ 7B w/o Calibration} & 0.092 & 75.2\% & 0.062 & 83.8\% & 0.097 & 27.7\% & 0.137 & 29.8\% \\
     Distill\textsubscript{ 7B w/ Label Smoothing} & 0.096 & 74.5\% & 0.033 & 83.3\% & 0.041 & 29.2\% & 0.142 & 29.8\% \\
     Distill\textsubscript{ 7B w/ COD} & \textbf{0.050} & \textbf{77.2\%} &\textbf{ 0.027} & \textbf{84.7\%} & \textbf{0.029} & \textbf{30.5\%} & \textbf{0.082} & \textbf{30.8\%} \\
     Compare to w/o calibration& $\red{\uparrow_{4.2\%}}$ & $\red{\uparrow_{2.0\%}}$ & $\red{\uparrow_{3.5\%}}$ & $\red{\uparrow_{0.9\%}}$ & $\red{\uparrow_{6.8\%}}$ & $\red{\uparrow_{2.8\%}}$ & $\red{\uparrow_{5.5\%}}$ & $\red{\uparrow_{1.0\%}}$\\

    \bottomrule
    % & \multicolumn{10}{c}{\textbf{Forgetting}}
    % & 
    \end{tabular}

\end{table*}
% $\red{\uparrow}$ means the improvement of distilled models over fine-tuned small models.

==> Tables/main_result.tex <==
\begin{table*}[!t]
\footnotesize
\centering
    % \vskip 0.15in
    \begin{tabular}{l|cccc|cccc}
    \toprule

     
     & \multicolumn{4}{c}{\textsc{\textbf{In-Domain}}} & \multicolumn{4}{c}{\textsc{\textbf{Out-of-Domain}}} \\
     
     &\multicolumn{2}{c}{Commonsense QA}& \multicolumn{2}{c}{BoolQ} &\multicolumn{2}{c}{Alpaca $\rightarrow$ Commonsense QA}& \multicolumn{2}{c}{Alpaca $\rightarrow$ OBQA}\\
     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
      & ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ \\
      \midrule
     & \multicolumn{8}{c}{\textsc{Llama 1 : 33B $\rightarrow$ 7B}}\\
     \midrule
     Pre-train\textsubscript{ 7B} & 3 & 26.9 & 42.5 & 61.2 & 3 & 26.9 & 2.8 & 29 \\
     Teacher\textsubscript{ 33B} & 10.2 & 82.4 & 7.7 & 89.7 & 18.6 & 69.2 & 20.2 & 64.4 \\
     Fine-tune\textsubscript{ 7B} & 11.8 & 79.9 & 6.5 & 82.5 & 12.5 & 48.2 & 21.9 & 43.4 \\
     Distill\textsubscript{ 7B} & 9.4 & 78.9 & \textbf{4.0} & 85.3 & 5.3 & 43.1 & 18.1 & 39.8 \\
     FIRST\textsubscript{ 7B w/ Label Smoothing} & 9.1 & 78.1 & 19.0 & 85.3 & 5.2 & 43.9 & 19.0 & 37.6 \\
     FIRST\textsubscript{ 7B w/ Temperature Scaling} & \textbf{2.9} & \textbf{80.8} & \textbf{4.0} & \textbf{85.7} & \textbf{4.6} & \textbf{50.0} &\textbf{7.1} & \textbf{47.2} \\
     % COD to w/o Re-calibration& $\red{\uparrow_{6.5\%}}$ & $\red{\uparrow_{1.9\%}}$ & $\blue{\uparrow_{0\%}}$ & $\red{\uparrow_{0.4\%}}$ & $\red{\uparrow_{0.7\%}}$ & $\red{\uparrow_{6.9\%}}$ & $\red{\uparrow_{11\%}}$ & $\red{\uparrow_{7.4\%}}$\\
    
     \midrule
     & \multicolumn{8}{c}{\textsc{Llama 2 : 13B$^*$ $\rightarrow$ 7B}}\\
     \midrule
     Pre-train\textsubscript{ 7B} & 0.104 & 37.3\% & 0.392 & 57.8\% & 0.104 & 37.3\% & 0.114 & 44.6\% \\
     Pre-train\textsubscript{ 13B} & 0.066 & 51.1\% & 0.374 & 62\% & 0.066 & 51.1\% & 0.036 & 54.6\% \\
     Teacher\textsubscript{ 13B} & \gray{0.12} & \gray{81.6\%} & \gray{0.068} & \gray{89.7\%} & \gray{0.208} & \gray{65.7\%} & \gray{0.287} & \gray{58.3\%} \\
     Fine-tune\textsubscript{ 7B} & 0.14 & 76.8\% & 0.084 & 87.5\% & 0.212 & 50.0\% & 0.301 & 45.6\% \\
     Distill\textsubscript{ 7B w/o Re-calibration} & 0.109 & 80.0\% & 0.04 & 85.3\% & 0.077 & 50.9\% & 0.125 & 46.6\% \\
     Distill\textsubscript{ 7B w/ Label Smoothing} & 0.103 & \textbf{80.4\%} & 0.039 & 87.5\% & 0.075 & 51.1\% & 0.162 & 47.6\%\\
     Distill\textsubscript{ w/ COD} & \textbf{0.063} & 80.3\% & \textbf{0.014} & \textbf{87.9\%} & \textbf{0.055} & \textbf{51.4\%} & \textbf{0.081} & \textbf{49.5\%} \\
     COD to w/o Re-calibration& $\red{\uparrow_{4.6\%}}$ & $\red{\uparrow_{0.3\%}}$ & $\red{\uparrow_{2.6\%}}$ & $\red{\uparrow_{2.6\%}}$ & $\red{\uparrow_{2.2\%}}$ & $\red{\uparrow_{0.5\%}}$ & $\red{\uparrow_{4.4\%}}$ & $\red{\uparrow_{2.9\%}}$\\
     \midrule
     & \multicolumn{8}{c}{\textsc{OpenLlama : 13B $\rightarrow$ 7B}}\\
     \midrule
     Pre-train\textsubscript{ 7B} & 7.7 & 20.6 & 36 & 58.6 & 7.5 & 20.8 & 3.6 & 25.6 \\
     Pre-train\textsubscript{ 13B} & 8 & 33.7 & 38 & 59.3 & 8 & 33.7 & 4.7 & 35 \\
     Teacher\textsubscript{ 13B} & \gray{13.2} & \gray{78.5} & \gray{7.5} & \gray{87.6} & \gray{16.7} & \gray{49.5} & \gray{13.4} & \gray{50} \\
     Fine-tune\textsubscript{ 7B} & 10.5 & 75.0 & 3.6 & 81.5 & 21.6 & 28.3 & 16.1 & 30.4 \\
     Distill\textsubscript{ 7B w/o Re-calibration} & 9.2 & 75.2 & 6.2 & 83.8 & 9.7 & 27.7 & 13.7 & 29.8 \\
     Distill\textsubscript{ 7B w/ Label Smoothing} & 9.6 & 74.5 & 3.3 & 83.3 & 4.1 & 29.2 & 14.2 & 29.8 \\
     Distill\textsubscript{ 7B w/ COD} & \textbf{5} & \textbf{77.2} &\textbf{ 2.7} & \textbf{84.7} & \textbf{2.9} & \textbf{30.5} & \textbf{8.2} & \textbf{30.8} \\
     COD to w/o Re-calibration& $\red{\uparrow_{4.2\%}}$ & $\red{\uparrow_{2.0\%}}$ & $\red{\uparrow_{3.5\%}}$ & $\red{\uparrow_{0.9\%}}$ & $\red{\uparrow_{6.8\%}}$ & $\red{\uparrow_{2.8\%}}$ & $\red{\uparrow_{5.5\%}}$ & $\red{\uparrow_{1.0\%}}$\\

    \bottomrule
    % & \multicolumn{10}{c}{\textbf{Forgetting}}
    % & 
    \end{tabular}
    \caption{The overall experimental results of calibration and performance on downstream tasks under both in-domain and out-of-domain setting. We compare pre-trained models, fine-tuned teacher and student models, and distilled models w/ or w/o re-calibration. The $\uparrow$ represents the larger the better while the $\downarrow$ means the smaller the better. \textbf{Bold} represents the best among fine-tuned and distilled student models. \gray{Gray} represents the statistics presented are for reference only and should not be used for comparison purposes. The model sizes are all specified in the subscripts. $^*$: We use 13B teacher model for Llama 2 family as its 34B version is still not publicly available and its 70B version requires significantly more resources. }
    \label{tab:main_result}
    \vskip -0.2in

\end{table*}
% $\red{\uparrow}$ means the improvement of distilled models over fine-tuned small models.




==> Tables/omer_table.tex <==

\begin{table*}[!t]
\footnotesize
\centering
    % \vskip 0.15in
    \begin{tabular}{ll|cccc|cccc}
    \toprule
     
       &&\multicolumn{4}{c}{\textsc{\textbf{In-Domain}}} & \multicolumn{4}{c}{\textsc{\textbf{Out-of-Domain}}} \\
     
       &&\multicolumn{2}{c}{Commonsense QA}& \multicolumn{2}{c}{BoolQ} &\multicolumn{2}{c}{Alpaca $\rightarrow$ Commonsense QA}& \multicolumn{2}{c}{Alpaca $\rightarrow$ OBQA}\\
      &&ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ & ECE $\downarrow$ & Acc $\uparrow$ \\
      \midrule
       &&\multicolumn{8}{c}{\textsc{Llama 1 : 33B $\rightarrow$ 7B}}\\
     \midrule
      Pre-train\textsubscript{ 7B}&&0.042& 28.1\% & 0.425 & 61.3\% & 0.039 & 27.8\% & 0.04 & 27.2\% \\
      Fine-tune\textsubscript{ 7B}&&0.118& 79.9\%& 0.065& 82.5\%& 0.125& 48.2\%& 0.219& 43.4\%\\
      &\textsubscript{ 7B w/ COD}&\cellcolor{lightBlue}\textbf{0.029}&\cellcolor{lightBlue} \textbf{80.8\%}&\cellcolor{lightBlue} \textbf{0.04}&\cellcolor{lightBlue} \textbf{85.7\%}& \cellcolor{lightBlue}\textbf{0.046}& \cellcolor{lightBlue}\textbf{50.0\%}&\cellcolor{lightBlue} \textbf{ 0.071}& \cellcolor{lightBlue}\textbf{47.2\%}\\
      Distill&\textsubscript{ 7B w/o Re-calibration}&0.094 & 78.9\% & \textbf{0.04} & 85.3\% & 0.053 & 43.1\% & 0.181 & 39.8\% \\
      &\textsubscript{ 7B w/ Label Smoothing}&0.091 & 78.1\% & 0.190 & 85.3\% & 0.052 & 43.9\% & 0.19 & 37.6\% \\
 \multicolumn{2}{l}{Fine-tune Teacher\textsubscript{ 13B}}& \gray{0.102}& \gray{82.4\%}& \gray{0.077}& \gray{89.7\%}& \gray{0.186}& \gray{69.2\%}& \gray{0.202}&\gray{64.4\%}\\
    
     \midrule
       &&\multicolumn{8}{c}{\textsc{Llama 2 : 13B$^*$ $\rightarrow$ 7B}}\\
     \midrule
      Pre-train\textsubscript{ 7B}&&0.1 & 36.6\% & 0.386 & 57.2\% & 0.1 & 36.6\% & 0.125 & 44.7\% \\
      Fine-tune\textsubscript{ 7B}&&0.14 & 76.8\% & 0.084 & 87.5\% & 0.212 & 50.0\% & 0.301 & 45.6\% \\
     & \textsubscript{7B w/ COD}&\cellcolor{lightBlue} \textbf{0.063}& 80.3\%&\cellcolor{lightBlue} \textbf{0.014}&\cellcolor{lightBlue} \textbf{87.9\%}& \cellcolor{lightBlue}\textbf{0.055}& \cellcolor{lightBlue}\textbf{51.4\%}& \cellcolor{lightBlue}\textbf{0.081}&\cellcolor{lightBlue}\textbf{49.5\%}\\
      Distill&\textsubscript{ 7B w/o Re-calibration}&0.109 & 80.0\% & 0.04 & 85.3\% & 0.077 & 50.9\% & 0.125 & 46.6\% \\
      &\textsubscript{ 7B w/ Label Smoothing}&0.103 &\cellcolor{lightBlue} \textbf{80.4\%} & 0.039 & 87.5\% & 0.075 & 51.1\% & 0.162 & 47.6\%\\
      \multicolumn{2}{l}{Fine-tune Teacher\textsubscript{ 13B}}&\gray{0.12}& \gray{81.6\%}& \gray{0.068}& \gray{89.7\%}& \gray{0.208}& \gray{65.7\%}& \gray{0.287}& \gray{58.3\%}\\
     \midrule
       &&\multicolumn{8}{c}{\textsc{OpenLlama : 13B $\rightarrow$ 7B}}\\
     \midrule
      Pre-train\textsubscript{ 7B}&&0.075 & 20.8\% & 0.359 & 58.5\% & 0.075 & 20.8\% & 0.008 & 28.4\% \\
      Fine-tune\textsubscript{ 7B}&&0.105 & 75.0\% & 0.036 & 81.5\% & 0.216 & 28.3\% & 0.161 & 30.4\% \\
     & \textsubscript{ 7B w/ COD}&\cellcolor{lightBlue} \textbf{0.050}& \cellcolor{lightBlue}\textbf{77.2\%}& \cellcolor{lightBlue}\textbf{ 0.027}& \cellcolor{lightBlue}\textbf{84.7\%}&\cellcolor{lightBlue}\textbf{0.029}&\cellcolor{lightBlue} \textbf{30.5\%}& \cellcolor{lightBlue}\textbf{0.082}&\cellcolor{lightBlue}\textbf{30.8\%}\\
          Distill&\textsubscript{ 7B w/o Re-calibration}&0.092 & 75.2\% & 0.062 & 83.8\% & 0.097 & 27.7\% & 0.137 & 29.8\% \\
      &\textsubscript{ 7B w/ Label Smoothing}&0.096 & 74.5\% & 0.033 & 83.3\% & 0.041 & 29.2\% & 0.142 & 29.8\% \\
\multicolumn{2}{l}{Fine-tune Teacher\textsubscript{ 13B}}& \gray{0.132}& \gray{78.5\%}& \gray{0.075}& \gray{87.6}& \gray{0.167}& \gray{49.5\%}& \gray{0.134}&\gray{50\%}\\ 
    \end{tabular}


    \caption{The overall experimental results of calibration and performance on downstream tasks under both in-domain and out-of-domain setting. We compare pre-trained models, fine-tuned teacher and student models, and distilled models w/ or w/o re-calibration. The $\uparrow$ represents the larger the better while the $\downarrow$ means the smaller the better. \textbf{Bold} represents the best among fine-tuned and distilled student models. \gray{Gray} represents the statistics presented are for reference only and should not be used for comparison purposes. The model sizes are all specified in the subscripts. $^*$: We use 13B teacher model for Llama 2 family as its 34B version is still not publicly available and its 70B version requires significantly more resources. }
    \label{tab:main_result}
    \vskip -0.2in

\end{table*}
% $\red{\uparrow}$ means the improvement of distilled models over fine-tuned small models.





